Scene Adaptive Sparse Transformer for Event-based Object Detection

While recent Transformer-based approaches have shown impressive performances on event-based object detection tasks, their high computational costs still diminish the low power consumption advantage of event cameras. Image-based works attempt to reduce these costs by introducing sparse Transformers. However, they display inadequate sparsity and adaptability when applied to event-based object detection, since these approaches cannot balance the fine granularity of token-level sparsification and the efficiency of window-based Transformers, leading to reduced performance and efficiency. Furthermore, they lack scene-specific sparsity optimization, resulting in information loss and a lower recall rate. To overcome these limitations, we propose the Scene Adaptive Sparse Transformer (SAST). SAST enables window-token co-sparsification, significantly enhancing fault tolerance and reducing computational overhead. Leveraging the innovative scoring and selection modules, along with the Masked Sparse Window Self-Attention, SAST showcases remarkable scene-aware adaptability: It focuses only on important objects and dynamically optimizes sparsity level according to scene complexity, maintaining a remarkable balance between performance and computational cost. The evaluation results show that SAST outperforms all other dense and sparse networks in both performance and efficiency on two large-scale event-based object detection datasets (1Mpx and Gen1). Code: https://github.com/Peterande/SAST

==> sec/tab_fig/fig_architecture.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=2\columnwidth]{fig/Block_v3.pdf}
\caption{\textbf{Hierarchical architecture of the SAST.} Four SAST blocks containing SAST layers extract features from sparse tokens transformed from events.}
 \vspace{-3mm}
\label{fig_Architecture}
\end{figure*}

==> sec/tab_fig/fig_visualizations2.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig/visualization2.pdf}
\caption{Visualizations of (a) original events, (b) score heatmaps, and (c) selection results by using 2 different weighting methods. The two networks tend to select tokens corresponding to objects and outlines, respectively.}
 \vspace{-3mm}
\label{fig_visualizations2}
\end{figure}

==> sec/tab_fig/tab_ablation4.tex <==
\begin{table}[t]
  \centering
  \tabcolsep=0.06cm
  \begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}lcc|cc|c@{}}

      \cline{1-6}
      Spar. & $a$ \tiny$\times 10^{-3}$ & $p$
      & mAP (\%) & A-FLOPs (G) & runtime (ms) 
      \\
      \hline

      Lv.1 &1.25& 1.5
      & 47.2 & 4.2 & 20.7\\

      Lv.2 &1.25& 1.25
      & 48.2 & 2.7 & 20.3\\
      
      Lv.3 &1.0& 1.0
      & 48.2 & 2.4 & 19.7\\
      
      Lv.4 &1.25& 1.0
      & \textbf{48.3} & 1.8 & 19.7\\

      Lv.5 &1.5& 1.0
      & 46.8 & 1.5 & 19.5\\

      Lv.6 &1.25& 0.75
      & 46.9 & 1.2 & 18.9 \\

      Lv.7 &1.25& 0.5
      & 46.1 & 0.8 & 18.5\\
      

      

      

      

      \hline
    \end{tabular*}
  \end{adjustbox}
  \vspace{1mm}
  \caption{Detection performance on 1Mpx dataset. Selecting different values of $a$ and $p$ when calculating the initial scores $S_i$ and the $\text{L}p$ norm results in different network sparsity and performance. Performance does not continuously improve with increasing network sparsity, with the best performance observed at $a=1.25\times 10^{-3}$ and $p=1$.}
  \vspace{-3mm}
  \label{tab_ablsparse}%
\end{table}


==> sec/tab_fig/tab_video.tex <==

\begin{table}[h]
  \centering
  \tabcolsep=0.098cm
  \begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}l|cc|c@{}}

      \cline{1-4}
      Methods
      & mAP (\%) & A-FLOPs (G) %& runtime (ms) 
      & Params (M)
      \\
      \hline
      SAST
      & 48.8 & 6.0\ (2.2)
      & 18.9 \\
      \hline
    \end{tabular*}
  \end{adjustbox}
  \label{tab_video}%
\end{table}
